Semantic Instance Segmentation via Deep Metric Learning

We propose a new method for semantic instance segmentation, by first computing how likely two pixels are to belong to the same object, and then by grouping similar pixels together. Our similarity metric is based on a deep, fully convolutional embedding model. Our grouping method is based on selecting all points that are sufficiently similar to a set of "seed points", chosen from a deep, fully convolutional scoring model. We show competitive results on the Pascal VOC instance segmentation benchmark.

==> junk.tex <==
We show examples of mask
classification heatmaps in Fig. \ref{fig:ClassificationHeatmap}.
We see that most pixels inside the object make good seeds,
but pixels near the boundaries (e.g., on the legs of the cows)
are not so good.


==> kpm-results.tex <==
\section{Results}


  \begin{figure*}[!htbp]
\begin{centering}
\includegraphics[scale=0.27]{./figures/segment_overlay}
\par
\end{centering}

\caption{Example instance segmentation results from our method.
\label{fig:SegmentOverlay}
}
\end{figure*}

\input{APtable}


In this section, we discuss our experimental results.

 \subsection{Experimental Setup}

We follow the experimental protocol that is used by previous
state of the art methods
\cite{Liang2016,li2016fully,liang2015proposal,chen2015multi,Hariharan2014}.
In particular,
we train on the PASCAL VOC 2012 training
set, with additional instance mask annotation from
\cite{Hariharan2011},
and we evaluate on the PASCAL VOC 2012
validation set.

After training the model,
we compute a precision-recall curve for each class,
based on all the test data.
This requires a definition of what we mean by a true and false positive. We follow standard practice
and say that a predicted mask 
that has an intersection over union \iou\ with a true mask above
some threshold $\iouthresh$ (e.g. $50\%$)
is a true positive, unless the true mask is already detected, in which case the
detection is a false positive.
We provide results for three \iou\ thresholds: $\{0.5, 0.6, 0.7\}$ similar to previous work.
We then compute the area under the PR curve,
known as the ``average precision''  or \APr\ score
\cite{Hariharan2011}.
Finally, we average this over classes, to get the mean average
precision or \mAPr\ score.

We can also evaluate the quality of our method as a ``class agnostic'' region proposal generator.
There are two main ways to measure quality in this case.
The first is to plot the recall (at a fixed \iou) vs the number of
proposals.
The second is to plot the recall vs the \iou\ threshold
for a fixed number of proposals; the area under this curve is known as
the ``average recall'' or AR  \cite{Hosang2015}.
\eat{
We compute a separate such curve (and AR summary statistic) for each
number of proposals; to be comparable
with other works (e.g., \cite{Pinheiro2016,Hu2016}),
we will use $N \in \{10, 100, 1000\}$.
(We can also plot the recall at a fixed IoU threshold vs the number of
proposals.)
}


\subsection{Preprocessing}

We use the following data augmentation components during training:

\textbf{Random Rotation}: We rotate the training images by a random degree in the range of $[-10, 10]$.
 
\textbf{Random Resize}: We resize the input image during the training phase with a random ratio in the range of $[0.7, 1.5]$.

\textbf{Random Crop}: We randomly crop the images during the training phase. At each step, we randomly crop $100$ windows. 
We randomly sample one image weighted towards cropped windows that have more object instances inside.

\textbf{Random Flip}: We randomly flip our training images horizontally.





\subsection{Results on Pascal VOC 2012}

\begin{table}
\begin{centering}
\begin{tabular}{|c||c|c|c|c|c|c|}
\hline 
$\alpha$ & 0.1 & 0.2 & 0.3 & 0.4 & 0.5 & 0.6\tabularnewline
\hline 
\hline 
$mAP^{r}$ & 61.4 & 61.7 & \textbf{62.1} & 61.6 & 61.6 & 61.5\tabularnewline
\hline 
\end{tabular}
\par\end{centering}

\caption{We find out that the best performing $\alpha$ parameter for sampling
seed points is $0.3$. In the table, we compare the mAPr performance
for different values of $\alpha$.
\label{tab:AlphaSweep}
}
\end{table}


We first tried different values of $\alpha$ (which trades off diversity with
seediness when picking the next seed) to find the best performing seed
sampling strategy. The results are shown for different values of
$\alpha$ in Table \ref{tab:AlphaSweep}.
We use $\alpha=0.3$ in the rest of the paper.
We furthermore analyze the performance of our model given different
number of mask proposals (number of sampled seed points) in Table
\ref{tab:NumSampleSweep}. 
Our model reaches a $mAP^r$ performance of $59.7$ by only proposing
$10$ regions, which is only 2\% worse than when using 1000 samples.
In Table \ref{tab:NumSampleSweep}, we also show the  class
agnostic segment-level average recall for different number of mask
proposals.



\begin{table}
\tiny
\begin{centering}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline 
Number of samples & 10 & 20 & 30 & 40 & 50 & 60 & 70 & 80 & 90 & 100 & 200 & 500 & 1000\tabularnewline
\hline 
\hline 
AR at $50\%$ IOU & 55.8 & 58.5 & 61.0 & 63.0 & 65.2 & 66.7 & 68.4 & 69.8 & 70.8 & 71.9 & 77.4 & 82.2 & 83.6\tabularnewline
\hline 
$mAP^{r}$ with $\alpha=0.2$ & 59.7 & 60.7 & 60.7 & 60.9 & 61.2 & 61.3 & 61.1 & 61.1 & 61.0 & 61.0 & 61.4 & 61.5 & 61.7\tabularnewline
\hline 
\end{tabular}
\par\end{centering}

\caption{We analyze the performance of our model given the number of sampled
  seed points.
\label{tab:NumSampleSweep}
}

\end{table}

Figure~\ref{fig:SegmentOverlay} shows some qualitative results,
and
Table~\ref{tab:results_iou} shows our quantitative results.
In terms of mAP performance,
we rank 4th at 0.5 \iou\ threshold,
2nd at 0.6 \iou\ threshold,
and tied 3rd at 0.7 \iou\ threshold.
So our method is competitive, if not state of the art.

Regarding performance for individual classes,
we see that we do very well on large objects,
such as trains, dogs, and motorbikes,
but we do very poorly in the bicycle category.
(See Fig. \ref{fig:ClassificationHeatmap} for some examples.)
This is also true of the other methods.
The reason is that there is a large discrepancy between
the quality of the segmentation masks
in the training set of \cite{Hariharan2011}
compared to the PASCAL test set.
In particular, the training set uses a coarse mask covering the entire
bicycle, whereas the test set segments out each spoke of the wheels
individually.





